Inpaint4DNeRF: Promptable Spatio-Temporal NeRF Inpainting with Generative Diffusion Models

Current Neural Radiance Fields (NeRF) can generate photorealistic novel views. For editing 3D scenes represented by NeRF, with the advent of generative models, this paper proposes Inpaint4DNeRF to capitalize on state-of-the-art stable diffusion models (e.g., ControlNet) for direct generation of the underlying completed background content, regardless of static or dynamic. The key advantages of this generative approach for NeRF inpainting are twofold. First, after rough mask propagation, to complete or fill in previously occluded content, we can individually generate a small subset of completed images with plausible content, called seed images, from which simple 3D geometry proxies can be derived. Second and the remaining problem is thus 3D multiview consistency among all completed images, now guided by the seed images and their 3D proxies. Without other bells and whistles, our generative Inpaint4DNeRF baseline framework is general which can be readily extended to 4D dynamic NeRFs, where temporal consistency can be naturally handled in a similar way as our multiview consistency.

==> figs/qualitative5col.tex <==
\begin{figure*}[tp]
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/seed.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/another.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/init_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/warmup_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/final_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/view1.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/view2.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/init_rgb.png}
    \end{subfigure}
    \subcaption{``an old professor, standing''}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/warmup_rgb.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/oldprof/final_rgb.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/seed.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/another.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/init_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/warmup_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/final_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/view1.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/view2.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/init_rgb.png}
    \end{subfigure}
    \subcaption{``an Argentina soccer player''}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/warmup_rgb.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/soccershirt/final_rgb.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/seed.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/another.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/init_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/warmup_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/final_depth.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/view1.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/view2.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/init_rgb.png}
    \end{subfigure}
    \subcaption{``telegraph pole''}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/warmup_rgb.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/qual/pole/final_rgb.png}
    \end{subfigure}
    \hfill
\caption{qualitative results 3d. to be organized and completed. First row: seed image, another pre-processed image, depth maps. Second row: final renders of 2 views, rgb images of each training stage.}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

